Six-loop $\varepsilon$ expansion study of three-dimensional $n$-vector model with cubic anisotropy

The six-loop expansions of the renormalization-group functions of $\varphi^4$ $n$-vector model with cubic anisotropy are calculated within the minimal subtraction (MS) scheme in $4 - \varepsilon$ dimensions. The $\varepsilon$ expansions for the cubic fixed point coordinates, critical exponents corresponding to the cubic universality class and marginal order parameter dimensionality $n_c$ separating different regimes of critical behavior are presented. Since the $\varepsilon$ expansions are divergent numerical estimates of the quantities of interest are obtained employing proper resummation techniques. The numbers found are compared with their counterparts obtained earlier within various field-theoretical approaches and by lattice calculations. In particular, our analysis of $n_c$ strengthens the existing arguments in favor of stability of the cubic fixed point in the physical case $n = 3$.

==> cubic.tex <==
@Book{Vasilev2,
  Title                    = {Quantum field renormalization group in critical behavior theory and stochastic dynamics},
  Author                   = {Vasil'ev, A.~N.},
  Publisher                = {Chapman \& Hall/CRC},
  Year                     = {2004},
  Month                    = apr,
  Note                     = {originally published in Russian in 1998 by St.~Petersburg Institute of Nuclear Physics Press; translated by Patricia A.~de Forcrand-Millard},

  ISBN                     = {978-0-415-31002-4}
}

@Book{Vasilev,
  Title					   ={Quantum field renormalization group in critical behavior theory and stochastic dynamics},
  Author				  ={Vasil'ev, A.~N.},
  Year					  ={1998},
  Publisher               ={Petersburg Inst. Nucl. Phys., St. Petersburg},
  Note                    = {English transl.: The field theoretic renormalization group in critical behavior theory and stochastic dynamics, Chapman \& Hall/CRC, Boca Raton, 2004}
}


@Book{BogShirk2,
  Title                    = {Introduction to the theory of quantized fields},
  Author                   = {Bogoliubov, N.~N. and Shirkov, D.~V.},
  Editor                   = {Marshak, R.~E.},
  Publisher                = {Interscience Publishers},
  Year                     = {1959},

  Address                  = {New York},
  Note                     = {translated from Russian by G.~M.~Volkoff},
  Series                   = {Interscience monographs in physics and astronomy},
  Volume                   = {3}
}


@Book{BogShirk,
  Title					   ={Introduction to the theory of quantized fields},
  Author				  ={Bogoliubov, N.~N. and Shirkov, D.~V.},
  Year					  ={1976},
  Publisher               ={Nauka, Moskow},
  Note                    = {English transl.: Interscience, New York, 1980}
}

@article{WF72,
  title={},
  author={Wilson, K G and Fisher, M E},
  journal={Phys. Rev. Lett.},
  volume={28},
  number={},
  pages={240},
  year={1972},
  publisher={}
}

@article{AS94,
  title={},
  author={Antonenko, S A and Sokolov, A I},
  journal={Phys. Rev. B},
  volume={49},
  number={},
  pages={15901},
  year={1994},
  publisher={}
}

@article{K76,
  title={},
  author={Korzhenevskii, A L},
  journal={Zh. Eksp. Teor. Fiz.},
  volume={71},
  number={},
  pages={1434},
  year={1976},
  publisher={},
  note={ {Sov.} Phys. JETP 44 (1976) 751}
}

@article{AAh73,
  title={},
  author={A. Aharony},
  journal={Phys. Rev. B},
  volume={8},
  number={},
  pages={4270},
  year={1973},
  publisher={}
}

@article{W73,
  title={},
  author={Wallace, D},
  journal={J. Phys. C},
  volume={6},
  number={},
  pages={1390},
  year={1973},
  publisher={}
}

@article{TMVD02,
  title={},
  author={Tissier, M and Mouhanna, D and Vidal, J and Delamotte, B},
  journal={Phys. Rev. B},
  volume={65},
  number={},
  pages={140402},
  year={2002},
  publisher={}
}

@article{LP75,
  title={},
  author={Lyuksyutov, I F and Pokrovskii, V L},
  journal={Pis'ma v ZhETF},
  volume={21},
  number={},
  pages={22},
  year={1975},
  publisher={},
  note={{JETP} Lett. 21 (1975) 9}
  }


@article{FDC81,
  title={},
  author={Ferer, M and Van Dyke, JP and Camp, WJ},
  journal={Phys. Rev. B},
  volume={23},
  number={},
  pages={2367},
  year={1981},
  publisher={}
}

@article{NR82,
  title={},
  author={Newman, K E and Riedel, E K},
  journal={Phys. Rev. B},
  volume={25},
  number={},
  pages={264},
  year={1982},
  publisher={}
}



@article{KP17,
  title={},
  author={Kompaniets, M V and Panzer, E},
  journal={Phys. Rev. D},
  volume={96},
  number={},
  pages={036016},
  year={2017},
  publisher={}
}

@InProceedings{KompanietsPanzer:LL2016,
  title = {},
  Author                   = {Kompaniets, M.~V. and Panzer, E.},
  Booktitle                = {\href{http://pos.sissa.it/cgi-bin/reader/conf.cgi?confid=260}{Loops and Legs in Quantum Field Theory Leipzig, Germany, April 24--29}},
  Year                     = {2016},
  Note                     = {{PoS(LL2016)038}},
  Publisher                = {Proceedings of Science},

  Archiveprefix            = {arXiv},
  Eprint                   = {1606.09210},
  Primaryclass             = {hep-th},
 }

@Article{KalagovKompanietsNalimov:U(r),
  Title                    = {},
  Author                   = {{Kalagov}, G.~A. and {Kompaniets}, M.~V. and {Nalimov}, M.~Yu.},
  Journal                  = {Nucl. Phys. B},
  Year                     = {2016},

  Month                    = apr,
  Pages                    = {16},
  Volume                   = {905},
}  

@article{antonov2013critical,
  title={},
  author={Antonov, N V and Kompaniets, M V and Lebedev, N M},
  journal={J. Phys. A},
  volume={46},
  number={},
  pages={405002},
  year={2013},
  publisher={IOP Publishing}
}


@article{antonov2017critical,
  title={},
  author={Antonov, N V and Kompaniets, M V and Lebedev, N M},
  journal={Teor. Mat. Fiz.},
  volume={190},
  number={},
  pages={239},
  year={2017},
  publisher={Springer},
  note={{Theor. Math. Phys.} 190 (2017) 204.}
}

@Article{AdzhemyanKompaniets:5loopNumerical,
  Title                    = {Five-loop numerical evaluation of critical exponents of the {$\phi^4$} theory},
  Author                   = {Adzhemyan, L.~Ts. and Kompaniets, M.~V.},
  Journal                  = {J. Phys. Conf. Ser.},
  Year                     = {2014},
  Number                   = {1},
  Pages                    = {012049},
  Volume                   = {523},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2014JPhCS.523a2049A},
  Archiveprefix            = {arXiv},
  Booktitle                = {Proceedings of 15th International Workshop on Advanced Computing and Analysis Techniques in Physics Research (ACAT 2013)},
  Doi                      = {10.1088/1742-6596/523/1/012049},
  Eprint                   = {1309.5621},
  Fjournal                 = {Journal of Physics: Conference Series},
  Primaryclass             = {cond-mat.stat-mech},
  Slaccitation             = {%%CITATION = ARXIV:1309.5621;%%}
}

@Unpublished{BatkovichKirienkoKompanietsNovikov:GraphState,
  Title                    = {},
  Author                   = {{Batkovich}, D. and {Kirienko}, Y. and {Kompaniets}, M. and {Novikov}, S.},
  Note                     = {preprint, program repository: \url{https://bitbucket.org/mkompan/graph_state/downloads}},

  Month                    = sep,
  Year                     = {2014},

  Adsurl                   = {http://adsabs.harvard.edu/abs/2014arXiv1409.8227B},
  Archiveprefix            = {arXiv},
  Eprint                   = {1409.8227},
  Primaryclass             = {hep-ph},
  Slaccitation             = {%%CITATION = ARXIV:1409.8227;%%}
}

@article{KT95,
  title={},
  author={Kleinert, H and Thoms, S},
  journal={Phys. Rev. D},
  volume={52},
  number={},
  pages={5926},
  year={1995},
  publisher={}
}

@article{N89,
  title={},
  author={N. A. Shpot},
  journal={Phys. Lett. A},
  volume={142},
  number={},
  pages={474},
  year={1989},
  publisher={}
}


@article{S77,
  title={},
  author={A. I. Sokolov},
  journal={Fiz. Tverd. Tela},
  volume={19},
  number={},
  pages={747},
  year={1977},
  note={{Sov.} Phys. Solid State 19 (1977) 433}
}


@article{MS87,
  title={},
  author={Maier, I O and Sokolov, A I},
  journal={Izv. Akad. Nauk SSSR, Ser. Fiz.},
  volume={51},
  number={},
  pages={2103},
  year={1987},
  publisher={}
}

@article{BGZ74,
  title={},
  author={Bre\'zin, E and Le Guillou, J C and Zinn-Justin, J},
  journal={Phys. Rev. B},
  volume={10},
  number={},
  pages={893},
  year={1974},
  publisher={}
}

@article{KW73,
  title={},
  author={Ketley, I J and Wallace, D J},
  journal={J. Phys. A},
  volume={6},
  number={},
  pages={1667},
  year={1973},
  publisher={}
}
@article{MV98,
  title={},
  author={Mudrov, A I and Varnashev, K B},
  journal={Phys. Rev. E},
  volume={58},
  number={},
  pages={5371},
  year={1998},
  publisher={APS}
}

@article{DR79,
  title={},
  author={E. Domany, and  Riedel E K},
  journal={J. Appl. Phys.},
  volume={50},
  number={},
  pages={1804},
  year={1981},
  publisher={}
}

@article{YH77,
  title={},
  author={Yalabik, M C and Houghton, A},
  journal={Phys. Lett.},
  volume={61A},
  number={},
  pages={1},
  year={1977},
  publisher={}
}

@article{TN76,
  title={},
  author={Nattermann, T and Trimper, S},
  journal={J. Phys. A},
  volume={9},
  number={},
  pages={3337},
  year={1976},
  publisher={}
}

@article{NT75,
  title={},
  author={Nattermann, T and Trimper, S},
  journal={J. Phys. A},
  volume={8},
  number={},
  pages={2000},
  year={1975},
  publisher={}
}

@article{SAS97,
  title={},
  author={Shalaev, B N and Antonenko, S A and Sokolov, A I },
  journal={Phys. Lett. A},
  volume={230},
  number={},
  pages={105},
  year={1997},
  publisher={}
}

@article{MS88,
  title={},
  author={Maier, I O and Sokolov, A I},
  journal={Ferroelectrics Lett. Sect.},
  volume={9},
  pages={95},
  year={1988}
}

@article{B77,
  title={},
  author={G.A. Baker Jr.},
  journal={Phys. Rev. B},
  volume={15},
  number={},
  pages={1552},
  year={1977},
  publisher={}
}

@article{HL74,
  title={},
  author={Harris, A B and Lubensky, T C},
  journal={Phys. Rev. Lett.},
  volume={33},
  number={},
  pages={1540},
  year={1974},
  publisher={}
}

@article{L75,
  title={},
  author={Lubensky, T C},
  journal={Phys. Rev. B},
  volume={11},
  number={},
  pages={3573},
  year={1975},
  publisher={}
}

@article{J83,
  title={},
  author={G. Jug},
  journal={Phys. Rev. B},
  volume={27},
  number={},
  pages={609},
  year={1983},
  publisher={}
}

@article{MS84,
  title={},
  author={Maier, I O and Sokolov, A I },
  journal={Fiz. Tverd. Tela},
  volume={26},
  pages={3454},
  year={1984},
  note={{Sov.} Phys. Solid State 26 (1984) 2076}
}

@article{KS95,
  title={},
  author={Kleinert, H and Schulte-Frohlinde, V},
  journal={Phys. Lett. B},
  volume={342},
  number={},
  pages={284},
  year={1995},
  publisher={Elsevier}
}

@article{NK74,
  title={},
  author={Nelson, D R and Kosterlitz, J M and  Fisher, M E},
  journal={Phys. Rev. Lett.},
  volume={33},
  number={},
  pages={813},
  year={1974},
  publisher={APS}
}

@article{KTS97,
  title={},
  author={Kleinert, H and Thoms, S and Schulte-Frohlinde, V},
  journal={Phys. Rev. B},
  volume={56},
  number={},
  pages={14428},
  year={1997},
  publisher={APS}
}

@article{CPV00,
  title={},
  author={Carmona, J M and Pelissetto, A and Vicari, E},
  journal={Phys. Rev. B},
  volume={61},
  number={},
  pages={15136},
  year={2000},
  publisher={APS}
}

@article{HV11,
  title={},
  author={Hasenbusch, M and Vicary, E},
  journal={Phys. Rev. B},
  volume={84},
  number={},
  pages={125136},
  year={2011},
  publisher={}
}

@article{V00,
  title={},
  author={Varnashev, K B},
  journal={Phys. Rev. B},
  volume={61},
  number={},
  pages={14660},
  year={2000},
  publisher={APS}
}
@article{PS99,
  title={},
  author={Pakhnin, D V and Sokolov, A I},
  journal={Phys. Rev. B},
  volume={61},
  number={},
  pages={15130},
  year={2000},
  publisher={APS}
}

@article{PS01,
  title={},
  author={Pakhnin, D V and Sokolov, A I},
  journal={Phys. Rev. B},
  volume={64},
  number={},
  pages={094407},
  year={2001},
  publisher={APS}
}

@article{M89,
  title={},
  author={Mayer, I O},
  journal={J. Phys. A},
  volume={22},
  number={},
  pages={2815},
  year={1989},
  publisher={IOP Publishing}
}


@article{MSS89,
  title={},
  author = {Mayer, I O and Sokolov, A I and Shalayev, B N},
	journal = {Ferroelectrics},
	volume = {95},
	number = {},	
	pages = {93},
	year  = {1989},
	publisher = {},
}

@article{KS16,
  title={},
  author={Kudlis, A and Sokolov, A I},
  journal={Phys. Rev. E},
  volume={94},
  number={},
  pages={042107},
  year={2016},
  publisher={}
}

@article{FH00,
  title={},
  author={Folk, R and Holovatch, Yu and Yavors’kii, T},
  journal={Phys. Rev. B},
  volume={61},
  number={},
  pages={15114},
  year={2000},
  publisher={}
}

@article{BCK16,
  title={},
  author={Batkovich, D V and Chetyrkin, K G and Kompaniets, M V},
  journal={Nucl. Phys. B},
  volume={906},
  number={},
  pages={147},
  year={2016},
  publisher={}
}

@article{FHY00,
  title={},
  author={Folk, R and Holovatch, Yu and  Yavors’kii, T},
  journal={Phys. Rev. B},
  volume={62},
  number={},
  pages={12195},
  year={2000},
  publisher={}
}

@article{GZ98,
  title={},
  author={Guida, R and Zinn-Justin, J},
  journal={J. Phys. A},
  volume={31},
  number={},
  pages={8103},
  year={1998},
  publisher={}
}

@article{CH98,
  title={},
  author={Caselle, M and Hasenbusch, M},
  journal={J. Phys. A},
  volume={31},
  number={},
  pages={4603},
  year={1998},
  publisher={}
} 
@Comment{jabref-meta: databaseType:bibtex;}

@Unpublished{Vermaseren:NewFORM,
  Title                    = {New features of {FORM}},
  Author                   = {Vermaseren, J.~A.~M.},
  Note                     = {Website: \url{https://www.nikhef.nl/~form/}},

  Month                    = oct,
  Year                     = {2000},

  Adsurl                   = {http://adsabs.harvard.edu/abs/2000math.ph..10025V},
  Archiveprefix            = {arXiv},
  Eprint                   = {math-ph/0010025},
  Primaryclass             = {math-ph},
  Slaccitation             = {%%CITATION = MATH-PH/0010025;%%}
  
